Manifesto for Putting 'Chartjunk' in the Trash 2021!

In this provocation we ask the visualization research community to join us in removing chartjunk from our research lexicon. We present an etymology of chartjunk, framing its provocative origins as misaligned, and harmful, to the ways the term is currently used by visualization researchers. We call on the community to dissolve chartjunk from the ways we talk about, write about, and think about the graphical devices we design and study. As a step towards this goal we contribute a performance of maintenance through a trio of acts: editing the Wikipedia page on chartjunk, cutting out chartjunk from IEEE papers, and scanning and posting a repository of the pages with chartjunk removed to invite the community to re-imagine how we describe visualizations. This contribution blurs the boundaries between research, activism, and maintenance art, and is intended to inspire the community to join us in taking out the trash.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/recycling-bin.tex <==












% As a first step to removing chartjunk from our lexicon, we performed three actions:
% \begin{itemize}[nosep]
% \item editing 
% \item removing
% \item scanning
% \end{itemize}
% We offer these actions, exaggerated under the guise of performance, to the community as first steps in removing chartjunk from our lexicon. Editing is a public act of maintenance of the term's history. Removing is a material deletion of the term. And scanning is an invitation for future engagement. Through these performative actions, we take literal steps toward changing our community's use of the term.




% As a response to a term taken so seriously, we chose to utilize play and performance in our triptych performance of maintenance art. Maintenance art was a response crafted by 1970s art activist Mierle Laderman Ukeles when her role as a mother subsumed her identity as artist. She was the first artist-in-residence at NYC's Department of Sanitation and focused on depicting maintenance work as art. Her art(work) was tedious, like sweeping the streets of NYC as performance art, and shaking the hand of every garbage(wo)man, but it worked to highlight the necessity of maintenance and the invisible labor behind upkeep. It was through the act of maintenance, conceived as performance art, that Ukeles reframed the conversation around maintenance work. We, too, rely on maintenance art to reframe the conversation surrounding chartjunk, contributing our own performance and a triptych of digital artifacts as byproducts of our maintenance work.

% It is common place for authors to offer specific and actionable solutions, and yet, we felt that we could not offer a replacement term for chartjunk, given its ill-definition and embeddedness within our vernacular. Instead, we turn to performance and maintenance art as an initial ``solution." 

% I WILL COME BACK TO THIS @miriah
% Thus, our contribution to the community is our maintenance art, performed in three different ways: editing, removing, and scanning. Each is an act of maintenance that does the 

% Through editing 

% We offer these actions, exaggerated under the guise of performance, to the community as first steps in removing chartjunk from our lexicon. Editing is a public act of maintenance of the term's history. Removing is a material deletion of the term. And scanning is an invitation for future engagement. Through these performative actions, we take literal steps toward changing our community's use of the term.


% Through performance, we used literal the physical material instantion of chartjunk a physical material that we could quite literally maintain.


% As a first step to removing chartjunk from our lexicon, we performed three actions:
% \begin{itemize}[nosep]
% \item editing 
% \item removing
% \item scanning
% \end{itemize}
% We offer these actions, exaggerated under the guise of performance, to the community as first steps in removing chartjunk from our lexicon. Editing is a public act of maintenance of the term's history. Removing is a material deletion of the term. And scanning is an invitation for future engagement. Through these performative actions, we take literal steps toward changing our community's use of the term.

% And though these actions were ephemeral, completed as part of a performance, we present three artifacts, as opportunities for future engagements:
% % , that we lovingly call a triptych:
% \begin{itemize}[nosep]
% \item the edit 
% \item the video
% \item the scanned repository
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=6cm]{figures/website.png}
%     \caption{The triptych can be found online at \url{chartjunk.art}.}
% \end{figure}
% The artifacts are stored online at \url{chartjunk.art}. While a website design is not a contribution of this work, we were intentional about the aesthetic. Although the work is focused on maintenance, which implies an orderliness or cleanliness, we specifically chose to stay away from minimalist design since the work of maintenance is never finished. Even our use of a flaming garbage can as a favicon is an act of centering humor, a gentle reminder that we have taken a provocation too seriously. Within the website, each artifact can be found organized in folders. We invite you to explore the website as you read through the next subsections. Despite the artifacts spanning different mediums, each piece of the triptych is united by a dedication to playfully blurring the boundaries between research, activism, and maintenance art.



% \section{Call to action}
% At this point in our manifesto, we introduce a tone shift: more urgent, more radical. After a review of chartjunk's genealogy and our critique of its flaws, we hope that you're ready to join us as we throw out the trash. Specifically, we are advocating for our community to stop using the term.

% \subsection{Let's stop using it}
% By throwing out the trash, abandoning a term that we have demonstrated is imprecise, has negative connotations, and a history intertwined with bullying, we believe there will be the opportunity to create a new, more inclusive framework. 

% \begin{figure}
%     \centering
%     \includegraphics[width=6cm]{figures/scrap.png}
%     \caption{Remainders of the term chartjunk cut out from IEEE research papers.}
%     \label{fig:scraps}
% \end{figure}

% We have chosen to not offer a replacement term or terms because there is just too much that has been characterized under it. Instead, we make the recommendation that as researchers, we be more intentional with the words that we are using. What forms of epistemic violence are we committing by not taking the time to carefully question the history of the concepts that we use to communicate? Are there other words that we have taken for granted that require a deeper, closer look?

% To be clear, we are not advocating that we stop trying to do visualization research; instead, we're petitioning researchers to consider the wider consequences of using a loaded term. Let's be more precise with our vocabulary to understand the differences between a chart with harmful, misleading elements and a chart with visual elements that entice a viewer to engage with the visualization. 

% We invite readers to look through the \href{http://www.overleaf.com}{remnants of papers} that no longer have the term (it has been cut out). What are other words that can fill those gaps?

% So yes, maintenance is a drag. We spent time and energy collecting references, organizing this manifesto, tidying up \href{https://en.wikipedia.org/wiki/Chartjunk}{Wikipedia}, methodically (maybe neurotically) cutting out the term from many papers, leaving no word undusted, and there is more we can surely do ... for we're not even sure if we've managed to convince you, our hopeful ally, to take out the trash! 

% But as Mierle so eloquently said, ``after the revolution, who’s going to pick up the garbage on Monday morning?"

% \begin{flushright}We are.
% \end{flushright}


% \section{The Genealogy}
% \label{sect:facts}
% As part of our maintenance work, we present a genealogy of chartjunk. It is our intent, to hold on to our criticism until Section \ref{sect: trouble}. Do not be alarmed! We still want you, the reader, to throw out the junk. But as part of our protest, we invite you to critically read the presented history and engage with the written words as though we were tidying up in front of you. The following sections will be added to the \href{https://en.wikipedia.org/wiki/Chartjunk}{Wikipedia pag}e on chartjunk, July 30th, 2021. We do not know what will happen to our edits, but welcome revisions and further discussions as part our maintenance.

% \begin{figure}[h!]
%   \centering
%   \begin{subfigure}[b]{0.8\linewidth}
%     \includegraphics[width=\linewidth]{figures/preEdits.png}
%     \caption{Screen capture of the Wikipedia page before our edits. July 3, 2020.}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.8\linewidth}
%     \includegraphics[width=\linewidth]{figures/preEdits.png}
%     \caption{Screen capture of the Wikipedia page after our edits. July 3, 2020.}
%   \end{subfigure}
%   \caption{The initial Wikipedia page on chartjunk had little to no genealogy about the term's origin. We found that it also lacked clear characterization. It was in clear need of maintenance!}
%   \label{fig:coffee}
% \end{figure}
% \subsection{Characterization}
% In 1983, Edward Tufte coined the term chartjunk with its own dedicated chapter in his book \textit{The Visual Display of Quantitative Information}\cite{tufte2001}. The chapter begins with: ``The purpose of decoration varies [...] Regardless of its cause, it is all non-data-ink or redundant data-ink, and it is often chartjunk.'' This immediate characterization by Tufte is that chartjunk is not useful and distracts from the chart's main message: the data.

% % Tufte definition
% He goes on to characterize chartjunk into three different types:
% \begin{itemize}[noitemsep]
%     \item \textbf{unintentional optical art:} visual texture like gradients or stripes that add extra visual noise to a chart
%     \item \textbf{the dreaded grid}: grid lines
%     \item \textbf{the self-promoting graphical duck:} three-dimensional elements, infographical visual elements, other decorative elements
% \end{itemize}

% % How others interpret the term
% % Still no judgement
% While these are three categories presented in the book, chartjunk has also been interpreted by others in slightly varying ways. Such interpretations include ``all the parts of a visualization that do not convey data'' \cite{kosara2012} and ``nothing that supports the chart’s message in a meaningful way" \cite{few2011}. Additionally, in a study by Parsons and Shukla \cite{parsons2020}, the authors found that data visualization practitioners had ``little consensus on the definition of chartjunk, with a wide variety of interpretations.''

% % The minimalist principles of the term
% Although the characterizations of chartjunk vary, the design foundations are set in minimalist practice.

% \begin{quote}
%     ``Guidelines for good chart design often suggest that the addition of chartjunk, decorations and other kinds of non-essential imagery, to a chart can make interpretation more difficult and can distract readers from the data. This minimalist perspective advocates plain and simple charts that maximize the proportion of data-ink – or the ink in the chart used to represent data'' \cite{bateman2010}.
% \end{quote}

% Tufte's characterization and criticism of chartjunk relies on a preference toward minimalist design principles that increase the interpretability of data \cite{bateman2010}. 
% % ``The minimalist perspective argues that the inclusion of visual embellishments and correspondingly lower data-ink ratios in graphs decreases the interpretability of data” \cite{bateman2010}. 
% Minimalist design has been critiqued by scholars as a method to espouse objectivity, where no embellishment creates no bias and allows the data speak for themselves. However, scholars have noted that conventions of minimalism, or rather anti-decoration, are rhetorical devices that can be just as biased \cite{bateman2010, hill2016}.

% Discuss the benefits of chartjunk
% Yet, Tufte also states that chartjunk is useful at times

% \subsection{Contradictions}
% Chartjunk has been the subject of research since its inception. There are mixed results regarding how chartjunk impact the interpretation of a data visualization (see Borkin et al. \cite{borkin2013} for a review and introduction to the research). One of the first papers to study the effect of chartjunk was conducted by Bateman et al. in 2010 \cite{bateman2010}. Through a user study they compared highly decorated charts with minimalist charts. They found that not only did the chartjunk not affect the accuracy of interpreting the charts, but also proved to be more memorable after a few weeks.  

% In two studies, aimed at addressing the shortcomings of the Bateman research, Borkin et al. conducted an experiment to test whether charts with junk were more memorable than standard charts \cite{borkin2013}. They designed a crowd-sourced study where participants were shown many images briefly for 1 second each. If the image popped up again, the study participant would press a key to mark that they had seen it before. The images were an assortment of charts with and without chartjunk. At the end of their study, they found that ``visualizations with low data-to-ink ratios and high visual densities (i.e., more chartjunk and 'clutter') were more memorable than minimal, 'clean' visualizations'' \cite{borkin2013}. They concluded that ``novel and unexpected visualizations can be better remembered than the visualizations with limited variability that we are exposed to since elementary school.'' 

% In a follow-up study \cite{borkin2016}, addressing critiques about the experimental constructs \cite{few2013}, the authors extended the experiment by using eye tracking and exposing participants to the charts for a longer time period (10 seconds). This study confirmed the results of their earlier work: ``visualizations that were most recognizable after only 1 second of viewing also tend to be better described (after 10 second exposure).'' They observed that when study participants where trying to recognize whether they have seen a chart before, they spent more time trying to find something memorable when the chart had no chartjunk. Additionally, they found that semantically meaningful pictograms and redundant messaging (forms of chartjunk) did not hinder interpretation of charts, but rather increased understanding.

% In other studies, chartjunk has been shown to help users learn better. In a paper by Hullman et al. \cite{hullman2011}, the authors summarize psychological research about learning that supports the use of chartjunk in graphs. ``All learning requires encoding information, yet the differing degrees to which learners can constructively process incoming information (as opposed to passively absorbing it through listening or reading) has led to definitions of active processing as active, self-directed searching for meaning on the part of the learner.'' In their paper, the authors expand on the benefits of introducing visual difficulties (many of which would be called chartjunk) for the purposes of learning and end with implications for design and evaluation. In a more recent study, researchers focused on understanding how people with Intellectual and Developmental Disabilities (IDD) understood visualizations \cite{wu2021}. They found that chartjunk in the form of icons tended to help with comprehension. Similar to the results from Borkin et al.'s 2016 study, the researchers found that icons were useful when they were semantically meaningful and relevant to the individual and their experience: ``simple, meaningful imagery has the potential to support data access.''

% The above studies focused on understanding the effect of chartjunk on interpretability and memorability of data visualizations. Recently, Parsons and Shukla interviewed data visualization practitioners to understand how chartjunk was and was not used by their community \cite{parsons2020}. They reported that the term chartjunk was broad and hard to define specifically by the practitioners. They also found that some practitioners did not think about chartjunk ``not because they had particular opinions about their use, but because they thought of themselves as not being able to produce embellishments effectively.'' And finally, they found that although there is research published in the visualization community (through venues like IEEE) about when and how to use chartjunk, visualization practitioners seemed to use their own situated judgements over the research: 

% ``Our work shows that the ways in which practitioners use chartjunk in their practice are highly varied and pluralistic, being strongly influenced by personal characteristics and goals of designers, their underlying philosophies, and the situated and pragmatic aspects of the design setting.''\cite{parsons2020}
% ``Although findings from studies on chartjunk suggest when and how its use is appropriate (e.g., to increase memorability or engagement), these recommendations do not fully characterize the considerations that practitioners give towards its use.''\cite{parsons2020}



% \subsection{Controversy}
% The term chartjunk has sparked much debate and controversy surrounding whether such decorations are useful in visualizations. In \textit{Envisioning Information} \cite{tufte1990}, Tufte begins a debate with Nigel Holmes, calling his graphic ``unsavory'' and ``cliché,'' accusing Holmes of ``contempt for [his] audience, designing as if readers were obtuse and uncaring.'' Stephen Few presents a review of this debate, stating that: ``In Holmes’ mind, Tufte became his nemesis and ever after these titans came to embody two sides of a debate that has raged for years'' \cite{few2011}. In a 1990 New York Times article, discussing the tension between Holmes and Tufte, the author writes: ``Time's Nigel Holmes, creator of the diamonds graph, was understandably irked when Tufte criticized it. Holmes admits his work has sometimes been exaggerated, but feels that Tufte, in his insistence on absolute mathematical fidelity, remains trapped in 'the world of academia' and insensitive to 'the world of commerce,' with its need to grab an audience'' \cite{nyt1992}.

% % BATEMAN
% While it is unclear what happened between Tufte and Holmes in the years following, a new debate began within the information visualization community. Following the publication of Bateman et al., Stephen Few released an article on his blog, Perceptual Edge, about the shortcomings of the research \cite{few2011}. In the article, he reviewed the premise of the research and then criticized the following: 

% \begin{itemize}[noitemsep]
%     \item the external validity of the experiment
%     \item the limitations of using Holmes-style charts as representative of chartjunk
%     \item the ``ugly'' design of the non chartjunk charts
%     \item and other experimental conditions (e.g. sample population and other potential confounding factors)
% \end{itemize}
% % 1. The purpose for which the charts in the test were used is typical of the way quantitative graphs are
% used in the real world.
% 2. The embellished charts by Nigel Holmes’ represent extreme examples of chartjunk.
% 3. The plain charts were designed in the manner that proponents of graphical “minimalism” advocate.
% 4. A study involving 20 university students can produce trustworthy results.
% 5. This study identified relevant factors and adequately controlled them

% While the article itself criticized the paper, at the end of the paper, Few thanks Scott Bateman ``for graciously supporting [his] efforts to write this article'' calling him a ``fine researcher'' because of his ``openness to other perspectives.''

% “I want to thank Scott Bateman of the research team for graciously supporting my efforts to write this article. Though he surely knows that I am not a fan of chartjunk, he provided me with his research data and answered all of my questions, without reservation. This openness to other perspectives is a sign of a fine researcher.”

% BORKIN “What Makes a Visualization Memorable?”
% The first Few post attacking “What Makes a Visualization Memorable?” [few2013]
% The post itself was civil-ish. It didn’t attach Borkin as he did in the second post

% Following the publication of Borkin et al.'s paper, “What Makes a Visualization Memorable?” \cite{borkin2013}, Few posts a review of their work on his blog \cite{few2013}. Along similar lines as his critique of Bateman et al.'s paper, Few highlights experimental shortcomings, such as the length that participants were shown the visualization. He concludes the post with the following sentence: ``Despite the flaws in this study, just like the others that have preceded it, dozens of future studies will cite it as credible and people will make outlandish claims based on it, which has already begun in the media.'' There is a brief exchange between Michelle Borkin and Stephen Few in the comments section. 

% \begin{quote}
%     Dear Stephen,
    
%     I certainly do wish that you had a similar reaction to this work as you had to my 2011 paper. Your reference to the Heath brothers (who credit Malcolm Gladwell with the “stickiness” moniker) seems quite appropriate as they talk of the need for memorability in communicating important ideas. They use “stickiness” to describe the memorable end of the “spectrum of memorability”.
    
%     The formal research study done by my fellow researchers and me simply aims to understand what aspects of a visualization move it to the memorable end of the spectrum of memorability. I am hopeful that over time and in light of follow-on research on visualization effectiveness you will see the value of this work.
    
%     Sincerely,
%     Michelle Borkin 

% \end{quote}

% To which Few responds in a more lengthy matter"

% \begin{quote}
%     % Michelle,

%     % Thanks for responding. It would be helpful, however, if you would address the specific points that I made in my critique. Doing so could help all of us learn something. You’ll find that I am willing to revise my opinion if you can show that I’ve erred.
    
%     I have argued that your study does not actually do what you claim. Your study does not reveal anything about what makes a visualization memorable. 
%     % It does not in any way help us design visualizations more effectively, nor serve as an “essential step” in the process. It’s hard to imagine how the study, as designed, could have possibly done so. 
    
%     % At most, your study suggests that particular visual elements and attributes catch our attention immediately when a visualization appears for only a second. That doesn’t make the visualization memorable. It makes a particular element or attribute exhibited in the visualization memorable. Nothing about the information contained in the visualization is remembered. In what sense is it useful for something about a visualization that isn’t information to be remembered? More fundamentally, how could an artificial activity that allows a visualization to be seen for only a second apply to actual uses of visualization, which are meant to be read and interpreted, not perceived in an instant?
    
%     % I believe that you derived some benefit personally by doing this work. I hope so. I don’t believe that the study has contributed anything useful to the field of data visualization. Nevertheless, we can learn something useful by critiquing the work to understand why it failed. 
%     There is no shame in a research failure unless we fail to recognize and learn from it. 
%     % On the other hand, as we’ve observed in recent years, it is harmful to claim results that are unfounded. 
%     Some of the most cited infovis studies of the last few years have been some of the worst. Knowing that your intentions are good, I’m sure that you don’t want to be responsible for another false promotion of chartjunk as useful. 
%     % Now that your study has been released into the wild, you have a chance to prevent this problem, at least in part, by more clearly stating what your study actually reveals, if anything, and what it doesn’t.
% \end{quote}

% After Borkin publishes a follow-up study \cite{borkin2016}, Few publishes another blog post where the statements shift from commentary about the research to comments about her education \cite{few2015}.
% % The second Few post attacking d “Beyond Memorability: Visualization Recognition and Recall”  [few2015]
% ``I suspect that her studies of memorability were dysfunctional because she lacked the experience and training required to do this type of research. She is now an Assistant Professor at Northeastern University, teaching the next generation of students. I’m concerned that she will teach them to produce pseudo-science. This is a depressing cycle.'' His tone is addressed in the comment\footnote{An archive can be found here: \href{https://web.archive.org/web/20160315040731/http://sfew.websitetoolbox.com/post/information-visualization-research-as-pseudoscience-7813635}{web.archive.org}} thread. In response to accusations of aggression Few responds in the following manner:

% \begin{quote}
%     “Your opening comment illustrates one of the reasons why critiques like mine are rarely published: the information visualization community tends to accuse anyone who writes a negative critique of being "aggressive." In fact, there are no examples of aggression in my critique. I invite you to read my article again and then, if you still feel that I was "unnecessarily aggressive" in any way, please do me the kindness of providing examples.”
% \end{quote}

% \begin{quote}
%     “Regarding the statements that you have identified as aggressive, reading what you wrote highlights the fact that "aggression" is not easy to measure objectively.”
% \end{quote}

% His tone was even mentioned in another blog, \href{https://eagereyes.org/blog/2015/memorability-science-and-the-value-of-thinking-outside-the-box}{Eager Eyes} by Robert Kosara, a research scientist at Tableau Software. The blog post is about visualization research as a science, questioned by Few, but begins with a section called ``Why the Personal Attacks?.'' Kosara writes that although there are many authors on the paper, Few focuses his criticism on Borkin. 
% % ``But let’s get this out of the way first. The whole thing is centered on Michelle Borkin, even though the paper has eight authors.“
% He also points out that ``Steve has so far mostly singled out women for his criticisms'' and that the tone of Few's writing is unwarranted, ``criticism is clearly useful, and so is pointing out issues. But the tone and personal style of this are way over the line.''

% \todo{@MIRIAH, please add the rest of the genealogy here}

% , work that will require constant vigilance. 
% These artifacts represent a blurring of research and maintenance art. Maintenance art was a term first used by the performance artist Mierle Laderman Ukeles in order to blur the lines of maintenance and art; drawing attention to all the work it takes to upkeep a home and a city. Inspired by her work, we want to bring attention to all the work it takes to upkeep a careful lexicon. 
% In the words of Ukeles, ``Maintenance is a drag; it takes all the fucking time (lit.)'' \cite{ukeles2018}.







% \section{Maintenance is a drag}
% \begin{quote}
%     \textit{Maintenance is a drag; it takes all the fucking time (lit.)
%     The mind boggles and chafes at the boredom. The
%     culture confers lousy status on maintenance jobs=
%     minimum wages, housewives=no pay.}
    
%     - Mierle Laderman Ukeles~\cite{ukeles2018}
% \end{quote}

% In this piece, we will attempt to convince you, the reader, to take out the trash; a little bit of maintenance that (hopefully) will not be a drag. It has come to our attention that the term \textit{chartjunk} has stuck to our lexicons, like a pesky piece of stubborn gum beneath a classroom desk. Since its inception in 1983~\cite{tufte2001}, it is a term that is still used despite the fact that it's ... well ... junk. As part of our manifesto (or plea, depending on who you are as a reader) we present a triptych\footnote{All of which can be found online: \url{https://chartjunk.art}} in addition to this paper:

% \begin{itemize}
% \item   A video of the first author cutting out the term chart junk from all IEEE papers as protest of the term, a demonstration of the work behind maintenance. Maintenance as art, art as maintenance.
% \item  The scans of papers with the term chartjunk cut out. An invitation for creativity. An opportunity to fill in the blanks.
% \item An edit of the chart junk \href{https://en.wikipedia.org/wiki/Chartjunk}{Wikipedia page}; both another act of protest and performance.
% \end{itemize}

% The accompanying video and leading quote to this paper is inspired by 1970s art activist Mierle Laderman Ukeles. She was the first artist-in-residence at NYC's Department of Sanitation and focused on elevating the work surrounding maintenance as art. Her work was tedious, sweeping the streets of NYC as performance art, but someone had to do it. We also felt the need to put in the work to "clean up" after the trail of chart junk both literally through engagement of literal materiality \textit{and} literally through physical enactments of removing the words through tedious action. You can find a link of the video here.

% Our manifesto focuses on maintenance, but yet we are proposing the dumping of a term, how can those two objectives coexist? We believe that through maintaining a record of the term's genealogy, we can expose the associated issues and baggage. 

% So dear reader, we cannot make you stop using a term, but with this manifesto we hope to persuade you that it is time to take out the trash.
